Real-time Safety Index Adaptation for Parameter-varying Systems via Determinant Gradient Ascend

Safety Index Synthesis (SIS) is critical for deriving safe control laws. Recent works propose to synthesize a safety index (SI) via nonlinear programming and derive a safe control law such that the system 1) achieves forward invariant (FI) with some safe set and 2) guarantees finite time convergence (FTC) to that safe set. However, real-world system dynamics can vary during run-time, making the control law infeasible and invalidating the initial SI. Since the full SIS nonlinear programming is computationally expensive, it is infeasible to re-synthesize the SI each time the dynamics are perturbed. To address that, this paper proposes an efficient approach to adapting the SI to varying system dynamics and maintaining the feasibility of the safe control law. The proposed method leverages determinant gradient ascend and derives a closed-form update to safety index parameters, enabling real-time adaptation performance. A numerical study validates the effectiveness of our approach.

==> img/arm_test_plot.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=4.036in,
height=1.777in,
at={(0.677in,3.041in)},
scale only axis,
xmin=0.5,
xmax=11.5,
xtick={2,4,6,8,10},
xticklabels={{},{},{},{},{}},
ymin=-0.05,
ymax=1.1,
ylabel style={font=\color{white!15!black}},
ylabel={Feasibility Rate},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
legend style={at={(0.2,0.7)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=black, line width=1.0pt, mark size=2.5pt, mark=*, mark options={solid, black}]
 plot [error bars/.cd, y dir=both, y explicit, error bar style={line width=1.0pt}, error mark options={line width=1.0pt, mark size=6.0pt, rotate=90}]
 table[row sep=crcr, y error plus index=2, y error minus index=3]{%
1	1	0	0\\
2	1	0	0\\
3	1	0	0\\
4	1	0	0\\
5	1	0	0\\
6	1	0	0\\
7	1	0	0\\
8	1	0	0\\
9	1	0	0\\
10	1	0	0\\
11	1	0	0\\
};
\addlegendentry{Adapted}

\addplot [color=black, dashed, line width=1.0pt, mark size=2.5pt, mark=*, mark options={solid, black}]
 plot [error bars/.cd, y dir=both, y explicit, error bar style={line width=1.0pt}, error mark options={line width=1.0pt, mark size=6.0pt, rotate=90}]
 table[row sep=crcr, y error plus index=2, y error minus index=3]{%
1	1	0	0\\
2	0.995666666666667	0.00750555349946514	0.00750555349946514\\
3	0.986333333333333	0.0195021366350801	0.0195021366350801\\
4	0.989	0.0121243556529822	0.0121243556529822\\
5	0.973	0.0317647603485372	0.0317647603485372\\
6	0.922666666666667	0.0765919926188981	0.0765919926188981\\
7	0.929	0.0620241888298428	0.0620241888298428\\
8	0.831333333333333	0.138500300842032	0.138500300842032\\
9	0.632	0.262	0.262\\
10	0.636	0.270005555498401	0.270005555498401\\
11	0.34	0.358434094360456	0.358434094360456\\
};
\addlegendentry{Nominal}

\end{axis}

\begin{axis}[%
width=4.036in,
height=1.777in,
at={(0.677in,0.573in)},
scale only axis,
xmin=0,
xmax=12,
xtick={0,2,4,6,8,10,12},
xticklabels={{(1.0 1.0)},{(0.5 0.5)},{(0.5 0.4)},{(0.4 0.5)},{(0.4 0.4)},{(0.4 0.3)},{(0.3 0.4)},{(0.3 0.3)},{(0.3 0.2)},{(0.2 0.3)},{(0.2 0.2)}},
xticklabel style={rotate=45},
ymin=0,
ymax=2.4,
ylabel style={font=\color{white!15!black}},
ylabel={$\theta$},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
legend style={at={(0.2,0.3)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=blue, line width=1.0pt, only marks, mark size=2.5pt, mark=*, mark options={solid, blue}]
 plot [error bars/.cd, y dir=both, y explicit, error bar style={line width=1.0pt}, error mark options={line width=1.0pt, mark size=6.0pt, rotate=90}]
 table[row sep=crcr, y error plus index=2, y error minus index=3]{%
1	0.288075053881806	0.0582351789501511	0.0582351789501511\\
2	0.633852022242196	0.141792848718256	0.141792848718256\\
3	0.715331022359092	0.173349920951275	0.173349920951275\\
4	0.60314719039429	0.0467814121560165	0.0467814121560165\\
5	0.842760298422412	0.089555108027037	0.089555108027037\\
6	0.906013178941796	0.0299389526090049	0.0299389526090049\\
7	1.41855903491435	0.715510188511137	0.715510188511137\\
8	1.43360052446459	0.742458742640262	0.742458742640262\\
9	1.45119824260313	0.415237526161492	0.415237526161492\\
10	1.31879823429209	0.152919496846402	0.152919496846402\\
11	1.8904415258182	0.149960851736401	0.149960851736401\\
};
\addlegendentry{$\theta'$}

\end{axis}
\end{tikzpicture}%
